Full Surround Monodepth from Multiple Cameras

Self-supervised monocular depth and ego-motion estimation is a promising approach to replace or supplement expensive depth sensors such as LiDAR for robotics applications like autonomous driving. However, most research in this area focuses on a single monocular camera or stereo pairs that cover only a fraction of the scene around the vehicle. In this work, we extend monocular self-supervised depth and ego-motion estimation to large-baseline multi-camera rigs. Using generalized spatio-temporal contexts, pose consistency constraints, and carefully designed photometric loss masking, we learn a single network generating dense, consistent, and scale-aware point clouds that cover the same full surround 360 degree field of view as a typical LiDAR scanner. We also propose a new scale-consistent evaluation metric more suitable to multi-camera settings. Experiments on two challenging benchmarks illustrate the benefits of our approach over strong baselines.

==> figures/both_qualitative.tex <==


\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-rgb_7_04131fb1.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-rgb_7_89a852c0.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-rgb_7_0935301b.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-rgb_7_851143ac.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-rgb_7_2fff9472.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-rgb_7_570fd51a.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-inv_depth_7_fda4f2df.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-inv_depth_7_2bca48a2.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-inv_depth_7_40721199.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-inv_depth_7_ee4b9656.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-inv_depth_7_262042e2.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-inv_depth_7_9a32b507.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{DDAD}]{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-calc_normals_7_c7875beb.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-calc_normals_7_11c2267c.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-calc_normals_7_4d9ba474.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-calc_normals_7_338b1655.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-calc_normals_7_2ff0a179.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-calc_normals_7_8df871f3.png}
}
//
\subfloat{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-rgb_1_40020b22.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-rgb_1_58b133e3.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-rgb_1_be6332ab.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-rgb_1_b91f6249.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-rgb_1_ee63df59.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-rgb_1_404be6c3.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-inv_depth_1_fc5d9c74.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-inv_depth_1_e7a451aa.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-inv_depth_1_14718541.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-inv_depth_1_556ac75b.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-inv_depth_1_36184bc7.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-inv_depth_1_66474543.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{nuScenes}]{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-calc_normals_1_74bf4dcd.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-calc_normals_1_9194d541.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-calc_normals_1_2e9b09c7.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-calc_normals_1_7e5eaccc.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-calc_normals_1_b3d8e70b.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-calc_normals_1_a356d291.png}
}
\caption{\textbf{Self-Supervised depth estimation results} on the \emph{DDAD} and \emph{nuScenes} datasets using our proposed method, including surface normals calculated from the predicted depth maps.}
\label{fig:ddad_qualitative}
\end{figure*}


==> figures/ddad_non_overlapping.tex <==

\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/rgb.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/rgb.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/rgb.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/rgb_context_1.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/mask_1_0_0.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask2.png}
}
\caption{\textbf{Non-overlapping masks} calculated on the \textit{DDAD} dataset. \textbf{First and second rows:} Target and context frames. \textbf{Third row:} Temporal mask from context to target. \textbf{Fourth row:} Spatial mask from surrounding target images.}
\label{fig:non_overlapping_masks}
\end{figure}


==> figures/ddad_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb2b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb4b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb5b.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> figures/pd_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb2b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb4b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb5b.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> figures/pd_warps.tex <==

\begin{figure*}[t!]
\vspace{-5mm}
\begin{tabular}{cc}
\centering
\multirow{6}{*}{
\hspace{-3mm}
\subfloat[Camera locations on the vehicle.]{
\raisebox{-51mm}{\includegraphics[width=0.28\linewidth,trim=0 350 0 0, clip]{images/pd_6cams.png}}}}
\hspace{-5mm}
& 
\\
& 
\hspace{0.2mm}
\subfloat{
\textcolor{cyan}{\rule{1.93cm}{1mm}}
\textcolor{magenta}{\rule{1.92cm}{1mm}}
\textcolor{yellow}{\rule{1.92cm}{1mm}}
\textcolor{green}{\rule{1.92cm}{1mm}}
\textcolor{blue}{\rule{1.92cm}{1mm}}
\textcolor{red}{\rule{1.92cm}{1mm}}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth,height=1.0cm]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_5.png}
}
\vspace{-4.5mm}
\\ 
&
\setcounter{subfigure}{1}
\subfloat[\textbf{First row:} Input RGB images. \textbf{Second and third rows:} Synthesized views from temporal contexts (Equation~\ref{eq:warp_mono}) and the corresponding photometric losses. \textbf{Third and fourth rows:} Synthesized views from surrounding cameras (Equation~\ref{eq:warp_spatial}) and the corresponding photometric losses (both overlaid).]{
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_5.png}
}
\end{tabular}
\caption{\textbf{Examples of spatial and temporal image warping} on the \textit{DDAD}  dataset. (a) shows the location of all six cameras, and (b) depicts the RGB images for each camera, alongside the synthesized images using information from other viewpoints and their corresponding photometric losses.}
\label{fig:pd_warps}
\vspace{-5mm}
\end{figure*}


==> tables/both_scaling_small.tex <==

\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{0.3em}
\subfloat[DDAD]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono $-$ M
    & F
    & 0.184
    & 0.366
    & 0.448
    & 0.417
    & 0.426
    & 0.438
    \\
    Mono
    & F 
    & 0.139
    & 0.209
    & 0.236
    & 0.231
    & 0.247
    & 0.204
    \\
    \textbf{FSM}
    & F
    & \underline{0.131}
    & \underline{0.203}
    & \underline{0.226}
    & \textbf{0.223}
    & \textbf{0.240}
    & \underline{0.188}
    \\
    \midrule
    Mono
    & S
    & 0.143
    & 0.238
    & 0.265
    & 0.277
    & 0.276
    & 0.247
    \\
    \textbf{FSM}
    & S
    & 0.133
    & 0.212
    & 0.229
    & 0.231
    & \underline{0.246}
    & 0.194
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.133
    & 0.219
    & 0.246
    & 0.252
    & 0.259
    & 0.197
    \\
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.131}
    & 0.206
    & 0.228
    & 0.238 
    & 0.248
    & \underline{0.188}
    \\
    \textbf{FSM}
    & -
    & \textbf{0.130}
    & \textbf{0.201}
    & \textbf{0.224}
    & \underline{0.229}
    & \textbf{0.240}
    & \textbf{0.186}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[nuScenes]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono
    & F 
    & 0.214
    & 0.304
    & 0.388
    & 0.314 
    & 0.438 
    & 0.304 
    \\
    \textbf{FSM}
    & F
    & 0.198
    & 0.297
    & \textbf{0.350}
    & \textbf{0.289} 
    & \textbf{0.392}
    & \underline{0.240}
    \\
    \midrule
    Mono
    & S
    & 0.251
    & 0.403 
    & 0.546
    & 0.429 
    & 0.616 
    & 0.321 
    \\
    \textbf{FSM}
    & S
    & 0.200 
    & 0.337 
    & 0.448
    & 0.354 
    & 0.521 
    & 0.267 
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.208
    & 0.382
    & 0.510
    & 0.393
    & 0.595
    & 0.258
    \\ 
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.187} 
    & \underline{0.291}
    & 0.392
    & 0.311
    & 0.448
    & 0.235
    \\ 
    \textbf{FSM}
    & -
    & \textbf{0.186}
    & \textbf{0.287}
    & \underline{0.375}
    & \underline{0.296}
    & \underline{0.418}
    & \textbf{0.221}
    \\
    \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Depth estimation results on multi-camera datasets}, using \emph{FSM} relative to the single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{F} denotes per-frame median-scaling, and \emph{S} our proposed shared median-scaling. \emph{M} denotes the removal of masking (Sec.~\ref{sec:mask}), \emph{STC} the removal of spatio-temporal contexts (Sec.~\ref{sec:stc}), and \emph{PCC} the removal of pose consistency constraints (Sec.~\ref{sec:pcc}).}
\label{tab:both_scaling_small}
\vspace{-3mm}
\end{table}

==> tables/ddad_ablation.tex <==

\captionsetup[table]{skip=6pt}

\begin{table}[t!]
\vspace{-3mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccc}
\toprule
\textbf{Method} & \textbf{Sup.} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
SuperDepth~\cite{superdepth} 
& $S$ & 0.112 & 0.875 & 4.958 & 0.852 \\
Monodepth2~\cite{godard2019digging} 
& $M$ & 0.115 & 0.903 & 4.863 & 0.877 \\
Monodepth2~\cite{godard2019digging} 
& $S$ & 0.109 & 0.873 & 4.960 & 0.864 \\
\midrule
Monodepth2~\cite{godard2019digging} 
& $M+S$ & \textbf{0.106} & \textbf{0.818} & 4.750 & \textbf{0.874} \\
Ours & $STC$ & 0.112 & 0.767 & \textbf{4.705} & 0.864 \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Ablation experiments on DDAD}, to validate the various components and design choices of our proposed architecture.}
\label{table:ddad_ablation}
\vspace{-3mm}
\end{table}

==> tables/ddad_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono
& Indiv. 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
& 0.832
& 0.709
& 0.673
& 0.686
& 0.660
& 0.695
\\
\textbf{MultiCam}
& Indiv.
& 0.131
& 0.203
& 0.226
& 0.223
& 0.240
& 0.188
& 0.840
& 0.716
& 0.687
& 0.693
& 0.670
& 0.714
\\
\midrule
Mono
& Shared
& 0.143
& 0.227
& 0.253
& 0.264
& 0.263
& 0.236
& 0.828
& 0.623
& 0.582
& 0.509
& 0.530
& 0.558
\\
\textbf{MultiCam}
& Shared
& 0.133
& 0.212
& 0.239
& 0.241
& 0.256
& 0.194
& 0.837
& 0.673
& 0.639
& 0.600
& 0.585
& 0.683
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.133
& 0.219
& 0.246
& 0.252
& 0.259
& 0.197
& 0.830
& 0.627
& 0.599
& 0.552
& 0.554
& 0.674
\\
\textbf{MultiCam}
& ---
& 0.131
& 0.206
& 0.228
& 0.238 
& 0.248
& 0.188
& 0.831
& 0.669
& 0.650
& 0.594
& 0.587
& 0.687
\\
\bottomrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Standard)}}}} 
% & 01 & 0.139 & 3.023 & 13.835 & 0.234 & 22.782 & 0.832 & 0.937 & 0.970
% \\
% & 05 & 0.209 & 3.410 & 12.609 & 0.319 & 30.722 & 0.709 & 0.881 & 0.938
% \\
% & 06 & 0.236 & 3.827 & 12.097 & 0.344 & 33.294 & 0.673 & 0.860 & 0.928
% \\
% & 07 & 0.231 & 3.976 & 12.311 & 0.331 & 31.874 & 0.686 & 0.863 & 0.931
% \\
% & 08 & 0.247 & 3.776 & 11.449 & 0.354 & 33.996 & 0.660 & 0.850 & 0.925
% \\
% & 09 & 0.204 & 3.345 & 14.371 & 0.309 & 30.150 & 0.695 & 0.889 & 0.949
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Shared)}}}} 
% & 01 & 0.143 & 3.133 & 13.875 & 0.237 & 23.029 & 0.828 & 0.935 & 0.970
% \\
% & 05 & 0.227 & 3.624 & 13.545 & 0.365 & 30.685 & 0.623 & 0.840 & 0.917
% \\
% & 06 & 0.253 & 4.197 & 13.324 & 0.400 & 33.375 & 0.582 & 0.821 & 0.905
% \\
% & 07 & 0.264 & 4.103 & 14.038 & 0.419 & 31.827 & 0.509 & 0.778 & 0.890
% \\
% & 08 & 0.263 & 3.856 & 12.739 & 0.419 & 34.001 & 0.530 & 0.795 & 0.896
% \\
% & 09 & 0.236 & 4.235 & 16.729 & 0.386 & 30.137 & 0.558 & 0.814 & 0.911
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Standard)}}}} 
% & 01 & 0.135 & 2.841 & 13.850 & 0.230 & 23.378 & 0.832 & 0.939 & 0.972
% \\
% & 05 & 0.207 & 3.239 & 12.608 & 0.320 & 30.793 & 0.705 & 0.879 & 0.938
% \\
% & 06 & 0.231 & 3.648 & 11.928 & 0.341 & 33.092 & 0.676 & 0.862 & 0.931
% \\
% & 07 & 0.225 & 3.804 & 12.341 & 0.330 & 31.804 & 0.688 & 0.863 & 0.930
% \\
% & 08 & 0.240 & 3.525 & 11.277 & 0.350 & 33.776 & 0.667 & 0.854 & 0.928
% \\
% & 09 & 0.200 & 3.379 & 14.934 & 0.312 & 30.450 & 0.694 & 0.887 & 0.948
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Shared)}}}} 
% & 01 & 0.138 & 2.924 & 14.041 & 0.232 & 22.557 & 0.826 & 0.937 & 0.971
% \\
% & 05 & 0.218 & 3.363 & 13.172 & 0.351 & 30.966 & 0.655 & 0.848 & 0.923
% \\
% & 06 & 0.241 & 3.896 & 12.827 & 0.377 & 32.893 & 0.621 & 0.835 & 0.914
% \\
% & 07 & 0.249 & 3.761 & 13.289 & 0.384 & 32.133 & 0.580 & 0.818 & 0.908
% \\
% & 08 & 0.257 & 3.549 & 12.096 & 0.393 & 33.719 & 0.568 & 0.821 & 0.910
% \\
% & 09 & 0.205 & 3.629 & 15.419 & 0.334 & 30.211 & 0.668 & 0.865 & 0.936
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Aware)}}}} 
% & 01 & 0.137 & 3.027 & 14.220 & 0.237 & 22.596 & 0.821 & 0.934 & 0.970
% \\
% & 05 & 0.211 & 3.335 & 13.219 & 0.350 & 30.966 & 0.661 & 0.849 & 0.923
% \\
% & 06 & 0.231 & 3.844 & 12.860 & 0.375 & 32.893 & 0.639 & 0.835 & 0.912
% \\
% & 07 & 0.244 & 3.731 & 13.303 & 0.384 & 32.133 & 0.589 & 0.814 & 0.907
% \\
% & 08 & 0.247 & 3.512 & 12.140 & 0.390 & 33.719 & 0.584 & 0.824 & 0.910
% \\
% & 09 & 0.191 & 3.479 & 15.370 & 0.328 & 30.211 & 0.693 & 0.869 & 0.937
% \\

\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed spatio-temporal photometric loss (\textit{Multi}) relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_ddad}
\end{table*}





==> tables/ddad_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono $-$ M
& F
& 0.184
& 0.366
& 0.448
& 0.417
& 0.426
& 0.438
\\
Mono
& F 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
\\
\textbf{FSM}
& F
& \underline{0.131}
& \underline{0.203}
& \underline{0.226}
& \textbf{0.223}
& \textbf{0.240}
& \underline{0.188}
\\
\midrule
Mono
& S
& 0.143
& 0.238
& 0.265
& 0.277
& 0.276
& 0.247
\\
\textbf{FSM}
& S
& 0.133
& 0.212
& 0.229
& 0.231
& 0.246
& 0.194
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.133
& 0.219
& \underline{0.246}
& 0.252
& 0.259
& 0.197
\\
\textbf{FSM $-$ PCC}
& -
& \underline{0.131}
& 0.206
& 0.228
& 0.238 
& 0.248
& \underline{0.188}
\\
\textbf{FSM}
& -
& \textbf{0.130}
& \textbf{0.201}
& \textbf{0.224}
& \underline{0.229}
& \textbf{0.240}
& \textbf{0.186}
\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed \emph{FSM} approach relative to the standard single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling.}
\label{tab:depth_ddad_small}
\end{table}





==> tables/nuscenes_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& Indiv. 
& 0.248
& 0.315
& 0.304 
& 0.304 
& 0.417 
& 0.398
& 0.727
& 0.629
& 0.659
& 0.712 
& 0.594
& 0.603
\\
\textbf{MultiCam}
& Indiv.
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
& 0.748
& 0.643
& 0.670
& 0.731
& 0.620
& 0.631
\\
\midrule
Mono
& Shared
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
& 0.729
& 0.520
& 0.511
& 0.659 
& 0.497
& 0.508
\\
\textbf{MultiCam}
& Shared
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
& 0.754
& 0.574
& 0.567
& 0.687 
& 0.549
& 0.558
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
& 0.691
& 0.526
& 0.516
& 0.680
& 0.536
& 0.542
\\ 
\textbf{MultiCam}
& ---
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
& 0.736
& 0.602
& 0.576
& 0.710
& 0.592
& 0.606
\\
\bottomrule


\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using our proposed spatio-temporal photometric loss (\textit{Multi} relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_nuscenes}
\end{table*}





==> tables/nuscenes_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& F 
& 0.214
& 0.304
& 0.294 
& 0.304 
& 0.408 
& 0.368
\\
\textbf{FSM}
& F
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
\\
\midrule
Mono
& S
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
\\
\textbf{FSM}
& S
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
\\ 
\textbf{FSM $-$ PCC}
& -
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
\\ 
\textbf{FSM}
& -
& \textbf{0.186}
& \textbf{0.287}
& 0.296
& 0.221
& 0.418
& 0.375
\\
\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using FSM relative to the standard single-camera photometric loss. In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling. \emph{M} refers to the removal of self-occlusion masks, and \emph{STC} to the removal of spatio-temporal constraints.}
\label{tab:depth_nuscenes_small}
\end{table}





==> tables/table_rot_averaging.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
FSM & 0.133 & 2.817 & \textbf{13.598} & 0.837\\
FSM + PCC (trans only) & 0.132 & 2.826 &  13.805 & 0.836\\
FSM + PCC (rot only) & 0.131 & 2.766 & 13.694 & 0.835 \\
\midrule
\textbf{FSM + PCC} & \textbf{0.130} & \textbf{2.752} & 13.866  & \textbf{0.838} \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Pose ablation (PCC)} described in Section 3.3. Our method with and without different components of the pose constraint, results on \textbf{F}.}
\label{table:pose-constraint}
\end{table}
